MetaICL: Learning to Learn In Context

We introduce MetaICL (Meta-training for In-Context Learning), a new meta-training framework for few-shot learning where a pretrained language model is tuned to do in-context learning on a large set of training tasks. This meta-training enables the model to more effectively learn a new task in context at test time, by simply conditioning on a few training examples with no parameter updates or task-specific templates. We experiment on a large, diverse collection of tasks consisting of 142 NLP datasets including classification, question answering, natural language inference, paraphrase detection and more, across seven different meta-training/target splits. MetaICL outperforms a range of baselines including in-context learning without meta-training and multi-task learning followed by zero-shot transfer. We find that the gains are particularly significant for target tasks that have domain shifts from the meta-training tasks, and that using a diverse set of the meta-training tasks is key to improvements. We also show that MetaICL approaches (and sometimes beats) the performance of models fully finetuned on the target task, and outperforms much bigger models with nearly 8x parameters. Finally, we show that MetaICL is complementary to human-written instructions, and the best performance can be achieved by combining both approaches.

==> sections/05-outdated-raw-results.tex <==
\begin{table*}[t]
    \centering \footnotesize
    %\setlength{\tabcolsep}{0.5em}
    \begin{tabular}{
        l @{\hspace{2em}}
        ccccccc
        }
        \toprule
            Method &
            \main &
            \makecell[c]{Class \\ $\rightarrow$Class} & \makecell[c]{non-Class \\ $\rightarrow$Class} &
            \makecell[c]{QA \\ $\rightarrow$QA} &
            \makecell[c]{non-QA \\ $\rightarrow$QA} &
            \makecell[c]{non-NLI \\ $\rightarrow$NLI} &
            \makecell[c]{non-Para \\ $\rightarrow$Para} \\
        \midrule
            \multicolumn{8}{c}{\em All target tasks} \\
            0-shot              & 34.9 & 34.0 & 34.0 & 39.9 & 39.9 & 25.7 & 36.5 \\
            PMI 0-shot          & 36.1 & 34.9 & 34.9 & 37.7 & 37.7 & 36.6 & 35.0 \\
            Channel 0-shot      & 40.0 & 42.4 & 42.4 & 40.4 & 40.4 & 31.4 & 37.3 \\
            In-context          & 36.5/34.7 & 36.0/33.2 & 36.0/33.2 & 39.6/38.4 & 39.6/38.4 & 26.4/25.6 & 33.1/33.1 \\
            PMI In-context      & 36.3/30.4 & 32.4/23.0 & 32.4/23.0 & 37.6/36.4 & 37.6/36.4 & 32.6/27.8 & 34.0/32.9 \\
            Channel In-context  & 42.0/36.9 & 45.2/38.4 & 45.2/38.4 & 40.2/37.6 & 40.2/37.6 & 39.4/33.3 & 44.4/41.7 \\
        \cmidrule{1-8}
            Multi-task 0-shot   & 41.9 & 37.4 & 36.9 & \textbf{45.3} & 35.6 & 42.4 & 36.7 \\
            Channel Multi-task 0-shot & 38.9 & 42.6 & 42.7 & 41.4 & 35.8 & 39.0 & 47.2 \\
            \ours               & 45.6/43.1 & 43.7/40.1 & 38.1/33.7 & 43.4/41.7 & 38.5/37.0 & \textbf{51.4}/48.1 & 35.1/33.2 \\
            Channel \ours       & \textbf{47.0}/43.0 & \textbf{47.1}/42.9 & \textbf{45.8}/40.9 & 41.2/38.5 & \textbf{40.3}/37.5 & 50.7/44.3 & \textbf{51.3}/47.9 \\
        \cmidrule{1-8}
            Oracle              & 46.4/40.0 & 50.7/44.0 & 50.7/44.0 & 41.8/39.1 & 41.8/39.1 & 44.3/32.8 & 54.7/48.9 \\
            Oracle w/ meta-train& 52.0/47.9 & 53.5/48.5 & 51.2/44.9 & 46.7/44.5 & 41.8/39.5 & 57.0/44.6 & 53.7/46.9 \\
        \toprule
            \multicolumn{8}{c}{\em Target tasks in unseen domains} \\
            0-shot              & 33.9 & 33.9 & 33.9 & 44.7 & 44.7 & 34.9 & 47.3 \\
            PMI 0-shot          & 24.5 & 24.5 & 24.5 & 22.8 & 22.8 & 49.7 & 37.1 \\
            Channel 0-shot      & 31.0 & 31.0 & 31.0 & 44.1 & 44.1 & 32.9 & 34.6 \\
            In-context          & 29.8/26.9 & 29.8/26.9 & 29.8/26.9 & 44.4/42.5 & 44.4/42.5 & 33.9/33.5 &34.1/ 34.1 \\
            PMI In-context      & 27.8/21.1 & 27.8/21.1 & 27.8/21.1 & 22.8/22.8 & 22.8/22.8 & 44.8/36.1 & 33.1/32.6 \\
            Channel In-context  & 37.5/31.3 & 37.5/31.3 & 37.5/31.3 & 45.4/40.0 & \textbf{45.4}/40.0 & 40.2/35.7 & 45.4/40.7 \\
        \cmidrule{1-8}
            Multi-task 0-shot   & 33.4 & 31.5 & 27.9 & \textbf{65.9} & 29.1 & 34.6 & 46.0 \\
            Channel Multi-task 0-shot & 32.1 & 27.7 & 33.3 & 51.6 & 42.8 & 59.4 & \textbf{53.5} \\
            \ours               & \textbf{41.1}/37.4 & 40.0/36.5 & 33.6/28.1 & 58.7/56.2 & 38.1/36.6 & \textbf{80.3}/77.7 & 42.0/34.4 \\
            Channel \ours       & 40.2/34.1 & \textbf{41.3}/36.7 & \textbf{41.4}/38.1 & 50.8/49.1 & 45.1/41.6 & 56.7/41.5 & 48.2/43.2 \\
        \cmidrule{1-8}
            Oracle              & 44.9/37.6 & 44.9/37.6 & 44.9/37.6 & 43.6/39.1 & 43.6/39.1 & 56.3/33.4 & 56.6/51.6 \\
            Oracle w/ meta-train& 53.3/43.2 & 53.2/43.7 & 46.1/36.9 & 67.9/66.2 & 44.5/42.8 & 71.8/58.2 & 65.6/61.4 \\
        \bottomrule
    \end{tabular}\vspace{-.3em}
    \caption{Main results, using GPT-2 Large.
    Two numbers indicate the average and the worst-case performance over different seeds used for $k$ target training examples.
    \textbf{Bold} indicates the best average result except oracle.
    `Class' indicates `Classification'.
    %\sewon{I ended up not including ensembling method which gives +2\% improvements in classification and less than 1\% improvements in others.}
    }\label{tab:main-result}
\end{table*}

\begin{table*}[t]
    \centering \footnotesize
    %\setlength{\tabcolsep}{0.5em}
    \begin{tabular}{
        l @{\hspace{1.5em}}
        ccccccc
        }
        \toprule
            Method &
            \main\ &
            \makecell[c]{Class \\ $\rightarrow$Class} & \makecell[c]{non-Class \\ $\rightarrow$Class} &
            \makecell[c]{QA \\ $\rightarrow$QA} &
            \makecell[c]{non-QA \\ $\rightarrow$QA} &
            \makecell[c]{non-NLI \\ $\rightarrow$NLI} &
            \makecell[c]{non-Para \\ $\rightarrow$Para} \\
        \midrule
            \multicolumn{8}{c}{\em All target tasks} \\
            Channel In-context  & 42.0/36.9 & 45.2/38.4 & 45.2/38.4 & 40.2/37.6 & 40.2/37.6 & 39.4/33.3 & 44.4/41.7 \\
            \ours               & 45.6/43.1 & 43.7/40.1 & 38.1/33.7 & 43.4/41.7 & 38.5/37.0 & \textbf{51.4}/48.1 & 35.1/33.2 \\
            Channel \ours       & \textbf{47.0}/43.0 & \textbf{47.1}/42.9 & \textbf{45.8}/40.9 & 41.2/38.5 & 40.3/37.5 & 50.7/44.3 & \textbf{51.3}/47.9 \\
        \cmidrule{1-8}
            GPT-J Channel In-context (x8) & 43.7/38.2 & 45.0/38.2 & 45.0/38.2 & \textbf{44.1}/41.3 & \textbf{44.1}/41.3 & 39.1/31.8 & 45.8/38.6 \\
        \toprule
            \multicolumn{8}{c}{\em Target tasks in unseen domains} \\
            Channel In-context  & 37.5/31.3 & 37.5/31.3 & 37.5/31.3 & 45.4/40.0 & 45.4/40.0 & 40.2/35.7 & 45.4/40.7 \\
            \ours               & \textbf{41.1}/37.4 & 40.0/36.5 & 33.6/28.1 & \textbf{58.7}/56.2 & 38.1/36.6 & \textbf{80.3}/77.7 & 42.0/34.4 \\
            Channel \ours       & 40.2/34.1 & \textbf{41.3}/36.7 & \textbf{41.4}/38.1 & 50.8/49.1 & 45.1/41.6 & 56.7/41.5 & \textbf{48.2}/43.2 \\
        \cmidrule{1-8}
            GPT-J Channel In-context (x8) & 40.5/35.3 & 40.5/35.3 & 40.5/35.3 & 47.9/43.8 & \textbf{47.9}/43.8 & 46.5/33.9 & {48.0}/45.0 \\
        \bottomrule
    \end{tabular}\vspace{-.3em}
    \caption{
    Comparison between raw LM in-context learning (based on GPT-2 Large and GPT-J) and \ours\ (based on GPT-2 Large). GPT-2 Large used unless otherwise specified.
    Two numbers indicate the average and the worst-case performance over different seeds used for $k$ target training examples.
    For raw LM baselines, Channel In-context is reported because it is the best raw LM baseline overall across the settings; full results based on GPT-J are provided in Appendix~\ref{app:results}.
    }\label{tab:comparison-gptj}
\end{table*}


\begin{table}[t]
    \centering \footnotesize
    %\setlength{\tabcolsep}{0.5em}
    \begin{tabular}{
        l @{\hspace{2em}} cc
        }
        \toprule
            Method &
            Diverse & No Diverse \\
        \midrule
            %\multicolumn{3}{c}{\em All target tasks} \\
            0-shot & \multicolumn{2}{c}{34.9} \\
            PMI 0-shot & \multicolumn{2}{c}{36.1} \\
            Channel 0-shot & \multicolumn{2}{c}{37.7} \\
            In-context & \multicolumn{2}{c}{36.5/34.7} \\
            PMI In-context & \multicolumn{2}{c}{36.3/30.4} \\
            Channel In-context & \multicolumn{2}{c}{42.0/37.3} \\
        \cmidrule{1-3}
            Multi-task 0-shot & 39.2 & 35.2 \\
            Channel Multi-task 0-shot & 40.1 & 37.2 \\
            \ours & \textbf{44.6}/41.7 & 37.6/34.3 \\
            Channel \ours & 44.3/40.5 & \textbf{42.1}/38.0 \\
        \bottomrule
    \end{tabular}\vspace{-.3em}
    \caption{Ablation on the diversity of meta-training tasks in the \main\ setting. For both settings, the number of meta-training tasks is 13, and the number of target tasks is 26 as in the original \main\ setting.
    A full list of meta-training tasks is shown in Appendix~\ref{app:dataset}.
    }\label{tab:ablate_diversity}
\end{table}

\begin{table}[t]
    \centering \footnotesize
    %\setlength{\tabcolsep}{0.5em}
    \begin{tabular}{
        l @{\hspace{0.6em}} c @{\hspace{1em}} c @{\hspace{1em}} c
        }
        \toprule
            Method &
            w/o Instruct & \multicolumn{2}{c}{w/ Instruct} \\
        \midrule
            \# instruct/task & 0 & 1 & 8.3 \\
        \midrule
            \multicolumn{4}{c}{\em All target tasks} \\
            0-shot &  33.3 & \multicolumn{2}{c}{34.7} \\
            PMI 0-shot & 33.1 & \multicolumn{2}{c}{38.5} \\
            Channel 0-shot & 33.2 & \multicolumn{2}{c}{30.2} \\
            In-context & 32.7/30.3 & \multicolumn{2}{c}{39.7/36.9} \\
            PMI In-context & 34.4/29.9 & \multicolumn{2}{c}{42.6/34.8} \\
            Channel In-context & 37.8/34.2 & \multicolumn{2}{c}{41.0/37.0} \\
        \cmidrule{1-4}
            MT 0-shot & 39.1 & 37.2 & 37.8 \\
            Channel MT 0-shot & 35.9 & 32.8 & 32.7 \\
            \ours & 37.0/34.2 & 43.2/40.0 & \textbf{45.3}/42.5 \\
            Channel \ours & 38.5/35.8 & 43.1/39.1 & 44.7/40.8 \\
        \toprule
            \multicolumn{4}{c}{\em Target tasks in unseen domains} \\
            0-shot &  33.9 & \multicolumn{2}{c}{29.5} \\
            PMI 0-shot & 24.5 & \multicolumn{2}{c}{32.8} \\
            Channel 0-shot & 31.0 & \multicolumn{2}{c}{30.3} \\
            In-context & 29.8/26.9 & \multicolumn{2}{c}{39.4/35.7} \\
            PMI In-context & 27.8/21.1 & \multicolumn{2}{c}{46.3/29.1} \\
            Channel In-context & 37.5/31.3 & \multicolumn{2}{c}{41.2/34.9} \\
        \cmidrule{1-4}
            MT 0-shot & 32.3 & 31.6  & 29.8 \\
            Channel MT 0-shot & 31.0 & 27.1  & 31.1 \\
            \ours & 31.5/26.8 & 47.0/43.2  & \textbf{49.3}/46.1 \\
            Channel \ours & 39.7/36.6 & 45.4/37.2  & 47.8/41.8 \\
        \bottomrule
    \end{tabular}\vspace{-.3em}
    \caption{Ablation on the impact of {\em natural instructions}.
    `w/ Instruct' uses instructions from \citet{sanh2021multitask}, either one per meta-training task or all available ones;
    `w/o Instruct' does not use instructions, as in all of our other experiments.
    `\# instruct/task' indicates the number of instructions per meta-training task on average.
    `MT 0-shot' indicates `Multi-task 0-shot' baselines.
    Both settings have the same meta-training and target tasks, %which numbers are
    32 and 12, respectively.
    %Note that `MT 0-shot' with instructions is equivalent to \citet{wei2021finetuned,sanh2021multitask}.
    A full list of tasks is shown in Appendix~\ref{app:dataset}.
    }\label{tab:ablate_inst}
\end{table}


\begin{table*}[t]
    \centering \footnotesize
    \setlength{\tabcolsep}{0.6em}
    \begin{tabular}{
        l @{\hspace{3em}} ccccc
        }
        \toprule
            Method & \main & 
            \makecell[c]{\{Class,non-Class\} \\ $\rightarrow$Class} & \makecell[c]{\{QA,non-QA\} \\ $\rightarrow$QA} &
            \makecell[c]{non-NLI \\ $\rightarrow$NLI} &
            \makecell[c]{non-Para \\ $\rightarrow$Para} \\
        \midrule
            \multicolumn{6}{c}{\em All tasks} \\
            0-shot & 37.9 & 35.1 & 45.0 & 25.4 & 33.3 \\
            PMI 0-shot & 43.6 & 38.6 & 41.8 & 36.6 & 36.1 \\
            Channel 0-shot & 39.7 & 35.8 & 42.5 & 27.6 & 41.8 \\
            In-context & 40.0/38.0 & 34.7/31.0 & \textbf{48.3}/46.2 & 26.9/25.4 & 33.1/33.1 \\
            PMI In-context & 40.1/36.3 & 35.1/29.0 & 42.0/40.7 & 31.0/25.3 & 34.7/33.4 \\
            Channel In-context & \textbf{43.7}/38.2 & \textbf{45.0}/38.2 & 44.1/41.3 & \textbf{39.1}/31.8 & \textbf{45.8}/38.6 \\
        \midrule
            \multicolumn{6}{c}{\em Target tasks in unseen domains} \\
            0-shot & 31.0 & 31.0 & 46.9 & 33.2 & 34.8 \\
            PMI 0-shot & 28.4 & 28.4 & 22.8 & 37.9 & 32.6 \\
            Channel 0-shot & 34.1 & 34.1 & \textbf{50.0} & 33.9 & 44.2 \\
            In-Context & 25.8/25.1 & 25.8/25.1 & 46.8/45.6 & 36.0/33.5 & 34.1/34.1 \\
            PMI In-Context & 25.4/20.1 & 25.4/20.1 & 22.8/22.8 & 33.2/33.2 & 34.1/34.1 \\
            Channel In-Context & \textbf{40.5}/35.3 & \textbf{40.5}/35.3 & 47.9/43.8 & \textbf{46.5}/33.9 & \textbf{48.0}/45.0 \\
        \bottomrule
    \end{tabular}\vspace{-.3em}
    \caption{Performance of raw LM baselines using GPT-J.
    Two numbers indicate the average and the worst-case accuracy over different seeds used for $k$ target training examples.
    `Class' indicate `Classification'.
    }\label{tab:full-result}
\end{table*}



\begin{table}[!ht]
    \centering \footnotesize
    %\setlength{\tabcolsep}{0.5em}
    \begin{tabular}{l @{\hspace{0.5em}} p{0.36\textwidth}}
        \toprule
            \em Single task \\
            Helpful: & tweet\_eval-offensive, glue-sst2, glue-mnli, wino\_grande, kilt\_hotpotqa \\
            Unhelpful: & race-middle, cosmos\_qa, dbpedia\_14,  gigaword, wikisql \\
        \midrule
            \em Task pair \\
            Helpful: &
            (yelp\_review\_full, glue-mnli), (yelp\_review\_full, wino\_grande),
            (hateexplain, glue-sst2),
            (hateexplain, glue-mnli),
            (hateexplain, glue-qqp),
            \\
            Unhelpful: &
            (paws, dbpedia\_14),
            (paws, art),
            (paws, cosmos\_qa),
            (cosmos\_qa, dbpedia\_14),
            (quail, art),
            \\
        \midrule
            \em Task triple \\
            Helpful &
            (yelp\_review\_full, glue-qqp, glue-mnli),
            (yelp\_review\_full, glue-sst2, glue-mnli),
            (yelp\_review\_full, hateexplain, glue-mnli),
            (yelp\_review\_full, hateexplain, qqp),
            (yelp\_review\_full, hate\_speech\_offensive, glue-mnli),
            \\
            Unhelpful &
            (paws, dbpedia\_14, art),
            (paws, dbpedia\_14, cosmos\_qa),
            (paws, cosmos\_qa, art),
            (dbpedia\_14, cosmos\_qa, art),
            (quail, paws, dbpedia\_14)
            \\
        \bottomrule
    \end{tabular}\vspace{-.3em}
    \caption{Analysis of which meta-training tasks give good performance in Channel \ours.
    We report five most helpful and the most unhelpful tasks (or task sets), respectively.}\label{tab:analysis_task}
\end{table}
